Scene as Occupancy

Human driver can easily describe the complex traffic scene by visual system. Such an ability of precise perception is essential for driver's planning. To achieve this, a geometry-aware representation that quantizes the physical 3D scene into structured grid map with semantic labels per cell, termed as 3D Occupancy, would be desirable. Compared to the form of bounding box, a key insight behind occupancy is that it could capture the fine-grained details of critical obstacles in the scene, and thereby facilitate subsequent tasks. Prior or concurrent literature mainly concentrate on a single scene completion task, where we might argue that the potential of this occupancy representation might obsess broader impact. In this paper, we propose OccNet, a multi-view vision-centric pipeline with a cascade and temporal voxel decoder to reconstruct 3D occupancy. At the core of OccNet is a general occupancy embedding to represent 3D physical world. Such a descriptor could be applied towards a wide span of driving tasks, including detection, segmentation and planning. To validate the effectiveness of this new representation and our proposed algorithm, we propose OpenOcc, the first dense high-quality 3D occupancy benchmark built on top of nuScenes. Empirical experiments show that there are evident performance gain across multiple tasks, e.g., motion planning could witness a collision rate reduction by 15%-58%, demonstrating the superiority of our method.

==> sections/introduction.tex <==
% !TEX root = ../egpaper_for_review.tex
\section{Introduction}
%------------------------------------------------------------------------
% challenge -> definition of 3D occupancy -> comparison -> value
Accurate 3D perception is challenging for autonomous driving (AD) systems due to the diverse entities present, from different vehicles to pedestrians, buildings, and vegetation, appealing to a unified, precise, and compact scene representation.
Quantizing the 3D scene into structured cells, with potentially semantic labels attached, is an intuitive solution, termed as \emph{3D Occupancy}.
Compared to traditional perception outputs such as 3D boxes, point cloud segmentation, and bird's-eye-view (BEV) segmentation, 3D occupancy can densely depict different objects and background shapes via the 3D cube collections with a good trade-off between accuracy and costs, as the construction vehicle with a crane arm shown in Fig.~\ref{fig:motivation}.
Therefore, exploring the potential of 3D occupancy as a scene representation to enhance traditional perception tasks and downstream planning is promising for this community.

As a scene representation, 3D occupancy does not come out of nowhere.
Occupancy grid map, a similar format in robotics, is a common representation in mobile navigation~\cite{moras2015grid}, but only serves as the search space of planning.
With the rapid advances of BEV perception in the past years, there is a renaissance of this representation, with more focus on its better perception granularity and generality.
MonoScene~\cite{cao2022monoscene} first explores using UNets to infer dense 3D occupancy with semantic labels from a single monocular RGB image, aka Semantic Scene Completion (SSC).
TPVFormer~\cite{huang2023tri} employs LiDAR-based sparse 3D occupancy as the supervision and proposes a tri-perspective-view (TPV) representation to aggregate features.
However, the community still seeks a practical approach to performing occupancy-based methods directly in the voxel space, better compatible with emerging BEV designs and more downstream tasks, and a playground to evaluate different representations in a full-stack autonomous driving pipeline, especially in the popular vision-centric solutions~\cite{yang2022goal}.

To this end, we propose \emph{OccNet}, an encoder-decoder occupancy network supporting multiple downstream tasks, and \emph{OpenOcc}, the first large-scale 3D occupancy dataset.
Specifically, unlike direct voxel feature construction from image features or sole use of BEV feature in previous works~\cite{li2022bevformer,chen2022persformer,wang2021depth}, \emph{OccNet} employs a cascade fashion to construct 3D occupancy feature from BEV feature effectively.
The decoder adopts a progressive scheme to recover the height information with voxel-based temporal and spatial cross-attention, composed of a deformable 3D attention module.
The resulting occupancy features can be then used for multiple downstream tasks without excessive computational overhead, including 3D occupancy prediction, 3D detection, BEV segmentation, and motion planning, serving as the framework foundation to evaluate different representations afterward.
%
To further provide the data foundation, we introduce \emph{OpenOcc} with dense and high-quality occupancy annotations.
It comprises 34149 annotated frames with over 1.4 billion 3D occupancy cells, each assigned to one of 16 classes to describe foreground objects and background stuff, and takes object motion into consideration with directional flow annotations.
%

Our empirical studies demonstrate the superiority of 3D occupancy as a scene representation over traditional alternatives from three aspects:
1) \emph{Dense is better.}
Dense 3D occupancy proves to be more effective than sparse forms in supporting 3D perception models. 
2) \emph{Better perception.}
3D occupancy facilitates the acquisition of 3D geometry from vision-only models, as evidenced by the point cloud segmentation performance comparable with LiDAR-based methods and the enhanced 3D detection performance with occupancy-based pre-training or joint training.
3) \emph{Better Planning.}
More accurate perception also translates into improved planning performance.
%
% \smch{stats result}
We evaluate OccNet on OpenOcc benchmark, outperforming the state of the art, e.g. TPVFormer~\cite{huang2023tri}, with the relative improvement of 14\% in semantic occupancy prediction task.
Compared with FCOS3D~\cite{wang2021fcos3d}, the detection model performance pre-trained on OccNet increase about 10 points when fine-tuned on small scale training data.
For the motion planning task based on occupancy feature, we can reduce the collision rate by 15\%-58\% compared with the planning policy based on BEV segmentation or 3D boxs. 


\iftrue
To sum up, our contribution comes into three folds: 
%
1) We propose OccNet, an encoder-decoder occupancy network that can easily suit current BEV methods and support multiple driving tasks with SoTA performance.
%
2) We propose OpenOcc, the first large-scale 3D occupancy benchmark with dense and high-quality annotations.
3) With an empirical analysis, we demonstrate that 3D occupancy is a better scene representation in the autonomous driving pipeline.
\fi

